Unveiling the Power of Deep Tracking

In the field of generic object tracking numerous attempts have been made to exploit deep features. Despite all expectations, deep trackers are yet to reach an outstanding level of performance compared to methods solely based on handcrafted features. In this paper, we investigate this key issue and propose an approach to unlock the true potential of deep features for tracking. We systematically study the characteristics of both deep and shallow features, and their relation to tracking accuracy and robustness. We identify the limited data and low spatial resolution as the main challenges, and propose strategies to counter these issues when integrating deep features for tracking. Furthermore, we propose a novel adaptive fusion approach that leverages the complementary properties of deep and shallow features to improve both robustness and accuracy. Extensive experiments are performed on four challenging datasets. On VOT2017, our approach significantly outperforms the top performing tracker from the challenge with a relative gain of 17% in EAO.

==> baseline.tex <==


\section{Baseline Approach}

%todo: Should be compressed. Consider moving to related work as a subsection. Have necessary equations inline. Only present the necessary stuff that we use later and refer to the paper for details.

%todo: Add motivation for why we use ECO as baseline

%With the state-of-the-art tracker C-COT as a baseline, we address the problem of deep feature utilization for visual tracking. DCF-based trackers alternate between parameter estimation and inference to predict the target location. The initial parameter estimation is done using the initial sample and the coresponding given bounding box. Subsequent parameter estimates are based also on earlier predictions.
We base our approach on the recently introduced Efficient Convolution Operator (ECO) \cite{DanelljanCVPR2017} method, shown to obtain state-of-the-art results while being computationally efficient. The ECO tracker aims at combining shallow and deep features by learning a multi-channel continuous convolution filter in a joint optimization scheme across all feature channels. Furthermore, it learns a projection matrix, which in essence is a $1\times 1$ convolution filter, to reduce the dimensionality of high-dimensional features. Here we briefly describe the training and inference procedures applied in the ECO tracker.

%We shall address feature utilization and argue that ECO merges different types of features in a naive and suboptimal way.

%Generally, the DCF-based framework alternates between learning, where model parameters are estimated; and inference, where the target location is estimated in a given video frame. In the initial learning phase, the tracker is given both a frame, and the target position. Subsequent parameter estimates are also based on earlier predictions.

The standard DCF-based framework learns the target model parameters based on a set of training samples and corresponding labels. We denote the set of training samples as $\{x_j\}_1^M$. Each training sample contains multiple feature layers $x_j^d\in\mathbb{R}^{N_d\times N_d}$, where $N_d$ is the spatial resolution of layer $d\in\{1,\dots,D\}$. Note that these multiple feature layers correspond to both shallow and deep features of varying resolutions. The corresponding set of labels $\{y_j\}_1^M$ are the desired detection scores, typically with a high value near the target center and mostly decaying to zero with increasing distance. The tracker predicts the target location using a learnt detection score operator, defined as
\begin{align}
  \label{eco_score}
  S_{f,P}\{x\} = \sum_{d=1}^Df^d*PJ_d\{x^d\} \,.
\end{align}
Here, $x$ is the input sample and $f$ is the estimated filter that produces scores for the target location. Note that $f$ is a multi-channel continuous convolution filter, with each channel $f^d\in L^2(T,T)$ being a Lebesgue integrable function of two variables. The convolution is denoted by $*$. The training samples are interpolated to the continuous domain using an interpolation operator $J_d$. In \eqref{eco_score} $P$ is a projection matrix applied to the training samples to reduce their dimensionality. For scale estimation, features are extracted at multiple scales, and the scale yielding the maximum detection score is selected as a target estimate. The detection score operator is learnt via minimization of
\begin{align}
  \label{eco_loss}
  E(f) = &\sum_{j=1}^M\alpha_j\|S_{f,P}\{x_j\}-y_j\|_{L^2}^2\nonumber\\
  &+ \sum_{d=1}^D\|wf^d\|_{L^2}^2 + \lambda^{\mathrm{proj}}\|P\|_2^2,
\end{align}
where the projection and filter are regularized by a constant $\lambda^{\mathrm{proj}}$ and spatial weighting, $w\in L^2(T,T)$ respectively. Each sample $x_j$ is weighted by $\alpha_j$, based on the learning rate $\gamma$. The labels $\{y_j\}_1^M$ are defined as
\begin{align}
  \label{label}
  y(t_1,t_2) = \expo{-\frac{(t_1-u_1)^2}{2(a\sigma)^2}}\expo{-\frac{(t_2-u_2)^2}{2(b\sigma)^2}},
\end{align}
periodically repeated. Here $(u_1,u_2)$ is the estimated target position. The variance of the Gaussian is controlled by the target size $(a,b)$ and a factor $\sigma$. Using Parseval's formula an equivalent discrete loss is obtained,
\begin{align}
  \label{eco_loss_fourier}
  E(f) =& \sum_{j=1}^M\alpha_k\|\widehat{S_{f,P}\{x_j\}}-\hat{y}_j\|_{\ell^2}^2\nonumber\\
  &+ \sum_{d=1}^D\|\hat{w}*\hat{f}^d\|_{\ell^2}^2 + \lambda^{\mathrm{proj}}\|P\|_2^2.
\end{align}
Here $\hat{\cdot}$ denotes the Fourier coefficients. This loss is approximated via truncation of the Fourier coefficients, resulting in a finite number of variables. These equations are efficiently solved using the method of Conjugate Gradients. For more details, we refer to \cite{DanelljanECCV2016,DanelljanCVPR2017}.

==> tables/otb_op.tex <==
\begin{tabular}{l@{~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}}
\toprule
&BACF&MCPF&ADNet&DeepSRDCF&MDNet&TCNN&C-COT&ECO&CREST&\textbf{Ours}\\\midrule
Mean OP&76.8&78.1&80.2&77.3&85.5&82.7&83.6&85&77.6&\textbf{88.1}\\\bottomrule
\end{tabular}

